GlanceNav: Efficient Vision-and-Language Navigation with Streaming Memory and Counterfactual Rewind

Multimodal large language models (MLLMs) have become strong policies for vision-and-language navigation (VLN). However, most of them encode a sample of past frames again at every decision and are trained on isolated decisions, so computation is redundant and the usable history is short. They also learn from their own mistakes through outcome rewards that give one scalar to a whole episode. We ask whether a navigator can encode each frame only once, at a constant cost per step, and still remember what matters and learn efficiently from its mistakes. We present GlanceNav, a streaming navigator built on a hybrid MLLM. Its Gated DeltaNet layers carry a recurrent state through the whole episode, while its attention layers keep a short window of recent observations and a small bank of keyframes, selected by how much each frame changes the recurrent state. This constant-size memory keeps the cost per step fixed and allows training on whole episodes with the same memory as at inference. Because the entire memory can also be copied in constant time, we further propose Counterfactual Rewind (CoRe), a reinforcement learning stage that rewinds a drifting rollout to its closest approach to the goal, lets an expert correct a few actions, and credits decisions by the resulting change in outcome. Trained only on the R2R-CE and RxR-CE training splits, with 1,000 instructions for reinforcement learning, a 4B GlanceNav reaches success rates of 71.9% and 73.6% on R2R-CE and RxR-CE val-unseen. On R2R-CE, it outperforms the strongest previous single-RGB method trained without external data by 9.1 points, while running at 104 ms per step.

==> fig/budget.tex <==
\begin{adjustbox}{max width=\linewidth}\begin{tikzpicture}[fig]
\pgfplotsset{budgetaxis/.style={scale only axis,
  width=3.2cm, height=3.7cm,
  xmin=3.2, xmax=12.8, xtick={4,6,8,12},
  xlabel={visible frames ($W{+}F$)},
  xlabel style={font=\sffamily\scriptsize,yshift=3pt},
  ylabel style={font=\sffamily\scriptsize,yshift=-4pt},
  tick label style={font=\sffamily\scriptsize,/pgf/number format/assume math mode=true},
  axis line style={inkC!55}, tick style={inkC!55},
  grid=major, grid style={black!7}, clip=false,
  title style={font=\sffamily\scriptsize\bfseries,yshift=-5pt}}}
\begin{axis}[budgetaxis, name=r2r,
  ymin=48.2, ymax=53.0, ytick={49,50,51,52,53},
  ylabel={SR (\%)}, title={(a) R2R-CE}]
\addplot[extC,line width=1pt,dash pattern=on 2.4pt off 1.2pt,mark=square*,mark size=1.5pt,mark options={solid}] coordinates {(4,48.72) (8,48.99) (12,51.22)};
\addplot[winC,line width=1pt,mark=triangle*,mark size=2.0pt] coordinates {(6,49.21) (8,52.42) (12,50.95)};
\addplot[ours,line width=1pt,mark=*,mark size=1.6pt] coordinates {(4,48.72) (6,50.84) (8,52.42) (12,51.33)};
\addplot[only marks,mark=*,mark size=1.6pt,inkC] coordinates {(4,48.72)};
\addplot[only marks,mark=*,mark size=2.3pt,mark options={fill=ours,draw=inkC,line width=0.6pt}] coordinates {(8,52.42)};
\node[text=ours!85!black,anchor=south west,inner sep=1.6pt] at (axis cs:8.25,52.42) {ours};
\end{axis}
\begin{axis}[budgetaxis, name=rxr, at={($(r2r.east)+(0.82cm,0)$)}, anchor=west,
  ymin=54.5, ymax=59.3, ytick={55,56,57,58,59},
  title={(b) RxR-CE}]
\addplot[extC,line width=1pt,dash pattern=on 2.4pt off 1.2pt,mark=square*,mark size=1.5pt,mark options={solid}] coordinates {(4,55.00) (8,55.30) (12,56.75)};
\addplot[winC,line width=1pt,mark=triangle*,mark size=2.0pt] coordinates {(6,56.23) (8,56.58) (12,56.01)};
\addplot[ours,line width=1pt,mark=*,mark size=1.6pt] coordinates {(4,55.00) (6,58.27) (8,56.58) (12,57.37)};
\addplot[only marks,mark=*,mark size=1.6pt,inkC] coordinates {(4,55.00)};
\addplot[only marks,mark=*,mark size=2.3pt,mark options={fill=ours,draw=inkC,line width=0.6pt}] coordinates {(8,56.58)};
\node[text=ours!85!black,anchor=south west,inner sep=1.6pt] at (axis cs:8.3,56.95) {ours};
\end{axis}
\begin{scope}[shift={($(r2r.south west)+(-0.35,-0.98)$)}]
  \draw[ours,line width=1pt] (0,0) -- (0.42,0); \fill[ours] (0.21,0) circle (1.6pt);
  \node[anchor=west,text=inkC,inner sep=1pt] at (0.48,0) {keyframes ($W{=}4$)};
  \draw[winC,line width=1pt] (2.95,0) -- (3.37,0);
  \fill[winC] (3.16,0.075) -- (3.085,-0.055) -- (3.235,-0.055) -- cycle;
  \node[anchor=west,text=inkC,inner sep=1pt] at (3.43,0) {window ($F{=}4$)};
  \draw[extC,line width=1pt,dash pattern=on 2.4pt off 1.2pt] (5.55,0) -- (5.97,0); \fill[extC] (5.71,-0.05) rectangle (5.81,0.05);
  \node[anchor=west,text=inkC,inner sep=1pt] at (6.03,0) {window only};
\end{scope}
\end{tikzpicture}\end{adjustbox}
\caption{\textbf{Spending the memory budget} (Stage~1, val-unseen SR; the models of \cref{tab:budget}). Orange: $W{=}4$ with $F{=}0,2,4,8$ keyframes. Blue: $F{=}4$ with $W{=}2,4,8$. Gray: no bank, $W{=}4,8,12$. Both panels span 4.8 points.}
\label{fig:budget}


==> fig/core_analysis.tex <==
\begin{adjustbox}{max width=\linewidth}\begin{tikzpicture}[fig]
\begin{axis}[name=sig,
  width=4.25cm,height=4.3cm,
  xmin=0.7,xmax=4.3,ymin=35,ymax=82,
  xtick={1,2,3,4},xticklabels={Q1,Q2,Q3,Q4},ytick={40,50,60,70,80},
  xlabel={quarter of training},ylabel={groups with a contrast (\%)},
  xlabel style={font=\sffamily\scriptsize,yshift=3pt},ylabel style={font=\sffamily\scriptsize,yshift=-5pt},
  tick label style={font=\sffamily\scriptsize,/pgf/number format/assume math mode=true},
  axis line style={inkC!55}, tick style={inkC!55},
  grid=major,grid style={black!7},clip=false,
  title={(a) Training signal},title style={font=\sffamily\scriptsize\bfseries,yshift=-5pt}]
\addplot[ours,line width=1.1pt,mark=*,mark size=1.6pt] coordinates {(1,76) (2,65) (3,64) (4,55)};
\addplot[stateC,line width=1.1pt,mark=square*,mark size=1.5pt] coordinates {(1,74) (2,61) (3,56) (4,53)};
\addplot[extC,line width=1.1pt,dash pattern=on 2.4pt off 1.2pt,mark=triangle*,mark size=1.9pt,mark options={solid}] coordinates {(1,64) (2,50) (3,40) (4,40)};
\node[text=ours!90!black,anchor=south west,inner sep=1pt] at (axis cs:2.15,67.0) {\core};
\node[text=stateC,anchor=center,inner sep=1pt] at (axis cs:3.28,49.6) {self-rewind};
\node[text=extC,anchor=center,inner sep=1pt] at (axis cs:3.5,43.6) {GRPO};
\end{axis}
\begin{axis}[name=out,at={($(sig.east)+(1.62cm,0)$)},anchor=west,
  width=4.2cm,height=4.3cm,
  xbar stacked,bar width=7.5pt,
  xmin=0,xmax=100,xtick={0,50,100},
  ymin=0.5,ymax=4.5,ytick={1,2,3,4},
  yticklabels={\core,Self-rewind,GRPO,Stage 2},
  y dir=reverse,
  xlabel={share of episodes (\%)},
  xlabel style={font=\sffamily\scriptsize,yshift=3pt},
  tick label style={font=\sffamily\scriptsize,/pgf/number format/assume math mode=true},
  axis line style={inkC!55}, tick style={inkC!55},
  axis x line*=bottom,axis y line*=left,
  title={(b) Where episodes end},title style={font=\sffamily\scriptsize\bfseries,yshift=-5pt},
  clip=false,
  after end axis/.code={
    \node[font=\sffamily\scriptsize,text=white] at (axis cs:34,1) {68.7};
    \node[font=\sffamily\scriptsize,text=white] at (axis cs:34,2) {67.3};
    \node[font=\sffamily\scriptsize,text=white] at (axis cs:32,3) {64.3};
    \node[font=\sffamily\scriptsize,text=white] at (axis cs:31.5,4) {63.7};
    \node[font=\sffamily\scriptsize,text=inkC] at (axis cs:85.3,1) {17.7};
    \node[font=\sffamily\scriptsize,text=inkC] at (axis cs:83.8,2) {19.6};
    \node[font=\sffamily\scriptsize,text=inkC] at (axis cs:83.8,3) {23.2};
    \node[font=\sffamily\scriptsize,text=inkC] at (axis cs:83.9,4) {27.0};
  }]
\addplot[fill=zeroC!85,draw=white,line width=0.3pt] coordinates {(68.73,1) (67.26,2) (64.33,3) (63.68,4)};
\addplot[fill=extC!60,draw=white,line width=0.3pt] coordinates {(7.72,1) (6.74,2) (7.88,3) (6.74,4)};
\addplot[fill=extC!24,draw=white,line width=0.3pt] coordinates {(17.67,1) (19.58,2) (23.16,3) (27.03,4)};
\addplot[fill=inkC!85,draw=white,line width=0.3pt] coordinates {(5.87,1) (6.42,2) (4.62,3) (2.56,4)};
\end{axis}
\begin{scope}[shift={($(sig.south west)+(0.35,-1.02)$)}]
  \fill[zeroC!85] (0,-0.07) rectangle (0.22,0.07); \node[anchor=west,text=inkC,inner sep=1pt] at (0.27,0) {success};
  \fill[extC!60] (3.2,-0.07) rectangle (3.42,0.07); \node[anchor=west,text=inkC,inner sep=1pt] at (3.47,0) {left the goal area};
  \fill[extC!24] (0,-0.36) rectangle (0.22,-0.22); \node[anchor=west,text=inkC,inner sep=1pt] at (0.27,-0.29) {never reached it};
  \fill[inkC!85] (3.2,-0.36) rectangle (3.42,-0.22); \node[anchor=west,text=inkC,inner sep=1pt] at (3.47,-0.29) {out of steps};
\end{scope}
\end{tikzpicture}\end{adjustbox}
\caption{\textbf{Why \core helps} (runs on 1k R2R-CE instructions, \cref{tab:core}). \textbf{(a)}~Share of instruction groups with an outcome contrast: main rollouts that differ in success, or a branch whose return differs from that of its main rollout. \textbf{(b)}~Outcome of all 1{,}839 R2R-CE val-unseen episodes, with the categories of \cref{fig:rl}b. \core mainly turns episodes that never came within 3\,m of the goal into successes.}
\label{fig:core_analysis}


==> fig/mask.tex <==
\begin{adjustbox}{max width=\linewidth}\begin{tikzpicture}[fig,x=1cm,y=1cm]
\def\cs{0.34}
\foreach \c/\h in {1/0.50,2/0.20,3/0.80,4/0.60,5/0.30,6/0.90,7/0.40,8/0.55,9/0.35}{
  \fill[stateC!45] ({\cs*\c-0.09},3.58) rectangle ({\cs*\c+0.09},{3.58+0.40*\h});
}
\node[text=stateC,anchor=east] at (0.12,3.72) {$\delta_s$};
\node[text=inkC] at (0,3.38) {$\pre$};
\foreach \c in {1,...,9}{\node[text=inkC] at ({\cs*\c},3.38) {\c};}
\foreach \r in {1,...,9}{
  \node[text=inkC,anchor=east] at (-0.22,{3.38-\cs*\r}) {$t{=}\r$};
  \foreach \c in {0,...,9}{
    \pgfmathtruncatemacro{\lo}{\r-2}
    \def\st{0}%
    \ifnum\c=0 \def\st{1}\fi
    \ifnum\c>0 \ifnum\c<\r \ifnum\c>\numexpr\lo-1\relax \def\st{2}\fi\fi\fi
    \ifnum\c=\r \def\st{3}\fi
    \ifnum\r=4 \ifnum\c=1 \def\st{4}\fi\fi
    \ifnum\r=5 \ifnum\c=1 \def\st{4}\fi\ifnum\c=2 \def\st{4}\fi\fi
    \ifnum\r=6 \ifnum\c=1 \def\st{4}\fi\ifnum\c=3 \def\st{4}\fi\fi
    \ifnum\r=7 \ifnum\c=3 \def\st{4}\fi\ifnum\c=4 \def\st{4}\fi\fi
    \ifnum\r=8 \ifnum\c=3 \def\st{4}\fi\ifnum\c=4 \def\st{4}\fi\fi
    \ifnum\r=9 \ifnum\c=3 \def\st{4}\fi\ifnum\c=6 \def\st{4}\fi\fi
    \pgfmathsetmacro{\xx}{\cs*\c}
    \pgfmathsetmacro{\yy}{3.38-\cs*\r}
    \ifcase\st
      \draw[black!10,fill=white,line width=0.3pt] (\xx-0.15,\yy-0.15) rectangle (\xx+0.15,\yy+0.15);
    \or \fill[extC!45] (\xx-0.15,\yy-0.15) rectangle (\xx+0.15,\yy+0.15);
    \or \fill[winC!40] (\xx-0.15,\yy-0.15) rectangle (\xx+0.15,\yy+0.15);
    \or \fill[winC!85] (\xx-0.15,\yy-0.15) rectangle (\xx+0.15,\yy+0.15);
    \or \fill[ours!70] (\xx-0.15,\yy-0.15) rectangle (\xx+0.15,\yy+0.15);
    \fi
  }
}
\node[text=inkC] at ({\cs*4.5},3.98+0.10) {key step};
\begin{scope}[shift={(3.85,2.95)}]
  \fill[extC!45] (0,0) rectangle (0.22,0.22); \node[anchor=west,text=inkC] at (0.28,0.11) {prefix $\pre$};
  \fill[ours!70] (0,-0.40) rectangle (0.22,-0.18); \node[anchor=west,text=inkC] at (0.28,-0.29) {keyframe bank (top-$F$ by $\delta$)};
  \fill[winC!40] (0,-0.80) rectangle (0.22,-0.58); \node[anchor=west,text=inkC] at (0.28,-0.69) {recent window};
  \fill[winC!85] (0,-1.20) rectangle (0.22,-0.98); \node[anchor=west,text=inkC] at (0.28,-1.09) {current step (causal)};
  \draw[black!10,line width=0.3pt] (0,-1.60) rectangle (0.22,-1.38); \node[anchor=west,text=inkC] at (0.28,-1.49) {not visible};
\end{scope}
\end{tikzpicture}\end{adjustbox}
\caption{\textbf{Attention mask of episode-level training} for one attention layer (schematic, $W{=}3$, $F{=}2$). Row $t$ shows the groups that step $t$ attends to. A group that leaves the window competes for the bank with its state-change score $\delta_s$ (top), so every row is known before the layer runs, and one forward pass trains all steps of the episode with the memory used at test time.}
\label{fig:mask}


==> fig/rl.tex <==
\begin{adjustbox}{max width=\linewidth}\begin{tikzpicture}[fig]
\begin{axis}[name=sig, scale only axis,
  width=2.72cm, height=2.3cm,
  xmin=0.45, xmax=4.4, ymin=24, ymax=84,
  xtick={1,2,3,4}, xticklabels={Q1,Q2,Q3,Q4}, ytick={30,40,50,60,70,80},
  xlabel={quarter of training}, ylabel={groups with a contrast (\%)},
  xlabel style={font=\sffamily\scriptsize,yshift=3pt}, ylabel style={font=\sffamily\scriptsize,yshift=-5pt},
  tick label style={font=\sffamily\scriptsize,/pgf/number format/assume math mode=true},
  axis line style={inkC!55}, tick style={inkC!55},
  grid=major, grid style={black!7}, clip=false,
  title={(a) Training signal}, title style={font=\sffamily\scriptsize\bfseries,yshift=-5pt}]
\addplot[ours,line width=1.1pt,mark=*,mark size=1.6pt] coordinates {(1,78) (2,63) (3,60) (4,59)};
\addplot[extC,line width=1.1pt,mark=triangle*,mark size=2.0pt,mark options={solid}] coordinates {(1,64) (2,50) (3,40) (4,36)};
\node[text=ours!85!black,anchor=south west,inner sep=1pt] at (axis cs:2.25,64.0) {\core};
\node[text=inkC,anchor=north east,inner sep=1pt] at (axis cs:2.72,42.0) {GRPO};
\node[text=ours!85!black,anchor=south,inner sep=2pt] at (axis cs:4,59) {59};
\node[text=inkC,anchor=north,inner sep=2.2pt] at (axis cs:4,36) {36};
\node[text=ours!85!black,anchor=west,inner sep=3.4pt] at (axis cs:1,78.8) {78};
\node[text=inkC,anchor=south west,inner sep=1.6pt] at (axis cs:1.05,64.3) {64};
\end{axis}
\begin{axis}[name=out, at={($(sig.east)+(1.38cm,0)$)}, anchor=west, scale only axis,
  width=2.78cm, height=2.3cm,
  xbar stacked, bar width=9.5pt,
  xmin=0, xmax=100, xtick={0,50,100},
  ymin=0.42, ymax=3.58, ytick={1,2,3},
  yticklabels={\core,GRPO,Stage 2},
  y dir=reverse,
  xlabel={share of episodes (\%)}, xlabel style={font=\sffamily\scriptsize,yshift=3pt},
  tick label style={font=\sffamily\scriptsize,/pgf/number format/assume math mode=true},
  axis line style={inkC!55}, tick style={inkC!55},
  axis x line*=bottom, axis y line*=left, clip=false,
  title={(b) Where episodes end}, title style={font=\sffamily\scriptsize\bfseries,yshift=-5pt},
  after end axis/.code={
    \node[text=white] at (axis cs:36,1) {71.9};
    \node[text=white] at (axis cs:33.5,2) {66.8};
    \node[text=white] at (axis cs:31.8,3) {63.7};
    \node[text=inkC] at (axis cs:86.95,1) {\fsS 17.5};
    \node[text=inkC] at (axis cs:84.5,2) {\fsS 20.3};
    \node[text=inkC] at (axis cs:83.9,3) {\fsS 27.0};
    \node[text=inkC,anchor=west,inner sep=1.5pt] at (axis cs:100,1) {\fsS 4.3};
    \node[text=inkC,anchor=west,inner sep=1.5pt] at (axis cs:100,2) {\fsS 5.4};
    \node[text=inkC,anchor=west,inner sep=1.5pt] at (axis cs:100,3) {\fsS 2.6};
  }]
\addplot[fill=zeroC!85,draw=white,line width=0.3pt] coordinates {(71.94,1) (66.83,2) (63.68,3)};
\addplot[fill=extC!60,draw=white,line width=0.3pt] coordinates {(6.25,1) (7.50,2) (6.74,3)};
\addplot[fill=extC!24,draw=white,line width=0.3pt] coordinates {(17.51,1) (20.28,2) (27.03,3)};
\addplot[fill=inkC!85,draw=white,line width=0.3pt] coordinates {(4.30,1) (5.38,2) (2.56,3)};
\end{axis}
\begin{scope}[shift={($(out.south west)+(-1.3,-0.84)$)}]
  \fill[zeroC!85] (0,-0.07) rectangle (0.22,0.07); \node[anchor=west,text=inkC,inner sep=1pt] at (0.27,0) {success};
  \fill[extC!60] (2.32,-0.07) rectangle (2.54,0.07); \node[anchor=west,text=inkC,inner sep=1pt] at (2.59,0) {left the goal area};
  \fill[extC!24] (0,-0.36) rectangle (0.22,-0.22); \node[anchor=west,text=inkC,inner sep=1pt] at (0.27,-0.29) {never reached it};
  \fill[inkC!85] (2.32,-0.36) rectangle (2.54,-0.22); \node[anchor=west,text=inkC,inner sep=1pt] at (2.59,-0.29) {out of steps};
\end{scope}
\end{tikzpicture}\end{adjustbox}
\caption{\textbf{Analysis of \core with 1{,}000 RL instructions} (runs of \cref{tab:rl}). \textbf{(a)}~Instruction groups with an outcome contrast: main rollouts that differ in success, or a branch whose return differs from that of its main rollout. \textbf{(b)}~Outcome of the 1{,}839 R2R-CE val-unseen episodes (goal area: within 3\,m).}
\label{fig:rl}


==> tab/budget.tex <==
\caption{\textbf{Memory budget} (Stage~1, val-unseen SR). Each row is a separately trained model. Frames: $W{+}F$, the frames visible to an attention layer. Plot: \cref{fig:budget}.}
\label{tab:budget}
\setlength{\tabcolsep}{6.2pt}
\footnotesize
\begin{adjustbox}{max width=\linewidth}\begin{tabular}{@{}l ccc cc@{}}
\toprule
Memory & $W$ & $F$ & Frames & R2R-CE & RxR-CE\\
\midrule
Window only & 4 & 0 & 4 & 48.7 & 55.0\\
 & 8 & 0 & 8 & 49.0 & 55.3\\
 & 12 & 0 & 12 & 51.2 & 56.7\\
\midrule
Window + bank & 2 & 4 & 6 & 49.2 & 56.2\\
 & 4 & 2 & 6 & 50.8 & \textbf{58.3}\\
\rowcolor{oursbg} & 4 & 4 & 8 & \textbf{52.4} & 56.6\\
 & 4 & 8 & 12 & 51.3 & 57.4\\
 & 8 & 4 & 12 & 51.0 & 56.0\\
\bottomrule
\end{tabular}\end{adjustbox}


==> tab/core.tex <==
\caption{\textbf{Ablation of \core} (R2R-CE val-unseen). RL uses 1{,}000 R2R-CE instructions; each entry is a single run. Bottom: SR for other trigger margins $\eta$ and expert horizons $H$.}
\label{tab:core}
\setlength{\tabcolsep}{5.2pt}
\footnotesize
\begin{adjustbox}{max width=\linewidth}\begin{tabular}{@{}l ccc@{}}
\toprule
Method & SR & SPL & OS\\
\midrule
GRPO, $G{=}4$~\cite{zhang2026activevln} & 64.3 & 57.3 & 72.4\\
GRPO, $G{=}5$ (same compute) & 66.5 & 58.7 & 75.2\\
\midrule
Self-rewind: the policy acts in the branch & 67.3 & 59.6 & 74.2\\
Branch at the trigger $t^\dagger$ & 66.7 & 57.3 & \textbf{76.9}\\
Imitate every correction & 67.0 & 59.3 & 76.3\\
No credit for the expert's actions & 64.9 & 57.7 & 74.6\\
\rowcolor{oursbg}\core{} ($\eta{=}1$\,m, $H{=}16$) & \textbf{68.7} & \textbf{60.9} & 76.7\\
\bottomrule
\end{tabular}\end{adjustbox}

\vspace{3pt}
\setlength{\tabcolsep}{5.6pt}
\begin{adjustbox}{max width=\linewidth}\begin{tabular}{@{}l ccc @{\hspace{14pt}} l ccc@{}}
\toprule
$\eta$ (m) & 0.5 & 1 & 2 & $H$ & 4 & 16 & 32\\
\midrule
SR & 67.1 & 68.7 & 65.8 & SR & 69.1 & 68.7 & 66.5\\
\bottomrule
\end{tabular}\end{adjustbox}


==> tab/memory.tex <==
\caption{\textbf{Selecting the bank} (Stage~1, R2R-CE val-unseen). Each row is a separately trained model with $W{=}4$. A bank holds the visual rows of four frames ($B{=}1{,}200$ rows) per attention layer: token rules keep the 1{,}200 highest-scoring visual rows, frame rules keep four whole frames. $e$, $v$, $\beta$: residual, value and write strength of \cref{eq:gdn}, averaged over heads unless noted. Cosine error: one minus the cosine between $v_i$ and its prediction by the state. Bottom: learned rankers.}
\label{tab:memory}
\setlength{\tabcolsep}{4.2pt}
\footnotesize
\begin{adjustbox}{max width=\linewidth}\begin{tabular}{@{}l l l cc@{}}
\toprule
Memory & Unit & Selection rule & SR & SPL\\
\midrule
Window only & -- & -- & 48.7 & 45.0\\
\midrule
Window + bank & token & $\beta\norm{e}$ (committed write~\cite{cui2026hippocampus}) & 51.7 & 48.4\\
 & token & $\norm{e}$ (prediction error) & 50.1 & 46.5\\
 & token & $(1{-}\beta)\norm{e}$ (unwritten error) & 50.7 & 47.4\\
 & token & $\beta\norm{v}$ & 50.4 & 46.9\\
 & token & $\norm{v}$ & 50.5 & 47.2\\
 & token & cosine error, min over heads & 49.9 & 46.7\\
 & token & cosine error, mean over heads & 49.0 & 45.4\\
 & frame & mean committed write over the frame & 49.3 & 45.5\\
 & frame & new-writes term of \cref{eq:decomp}, normalized as $\delta_s$ & 51.6 & \textbf{48.7}\\
\rowcolor{oursbg} & frame & state change $\delta_s$ of \cref{eq:delta} (ours) & \textbf{52.4} & \textbf{48.7}\\
\midrule
 & token & learned linear ranker & 51.7 & 48.2\\
 & token & learned MLP ranker & 50.7 & 47.2\\
\bottomrule
\end{tabular}\end{adjustbox}


==> tab/paradigm.tex <==
\caption{\textbf{Step-wise \vs episode-level training} of a Qwen3.5-4B navigator for one epoch on the same data (30.8K episodes, 3.13M actions). The step-wise model is the uniform-8 SFT model. Time: one epoch on four H100 GPUs.}
\label{tab:paradigm}
\setlength{\tabcolsep}{4pt}
\footnotesize
\begin{adjustbox}{max width=\linewidth}\begin{tabular}{@{}lcc@{}}
\toprule
 & Step-wise & \cellcolor{oursbg}Episode-level (ours)\\
\midrule
History per decision & 8 sampled frames & \cellcolor{oursbg}state + window + bank\\
Frames encoded per epoch & 27.0M & \cellcolor{oursbg}\textbf{3.13M}\\
Decisions per forward pass & 1 & \cellcolor{oursbg}\textbf{102}\\
Training time per epoch & 42.6\,h & \cellcolor{oursbg}\textbf{13.5\,h}\\
\midrule
R2R-CE SR / SPL & 46.5 / 42.3 & \cellcolor{oursbg}\textbf{52.4} / \textbf{48.7}\\
\bottomrule
\end{tabular}\end{adjustbox}


==> tab/randombank.tex <==
\caption{\textbf{Random \vs scored bank} under an earlier schedule (epoch-1 checkpoint of a two-epoch run; R2R-CE val-unseen). $B$: bank rows per attention layer.}
\label{tab:randombank}
\setlength{\tabcolsep}{4pt}
\footnotesize
\begin{adjustbox}{max width=\linewidth}\begin{tabular}{@{}l c r l cc@{}}
\toprule
Memory & $W$ & $B$ & Selection & SR & SPL\\
\midrule
Window only & 8 & 0 & -- & 46.3 & 41.8\\
Window only & 9 & 0 & -- & 43.5 & 40.2\\
Random bank & 8 & 300 & random & 46.1 & 43.4\\
Token bank & 8 & 300 & $\beta\norm{e}$ & 49.3 & 45.9\\
Random bank & 4 & 1{,}200 & random & 47.7 & 43.9\\
\rowcolor{oursbg}Token bank & 4 & 1{,}200 & $\beta\norm{e}$ & \textbf{51.0} & \textbf{47.4}\\
\bottomrule
\end{tabular}\end{adjustbox}


==> tab/rl.tex <==
\caption{\textbf{Training stages} (val-unseen). RL rows: one pass over 1{,}000 instructions from Stage~2, with the same instructions, order and seed for both methods.}
\label{tab:rl}
\setlength{\tabcolsep}{4.4pt}
\footnotesize
\begin{adjustbox}{max width=\linewidth}\begin{tabular}{@{}l cccc c@{}}
\toprule
 & \multicolumn{4}{c}{R2R-CE} & RxR-CE\\
\cmidrule(lr){2-5}\cmidrule(l){6-6}
Method & SR$\uparrow$ & SPL$\uparrow$ & OS$\uparrow$ & NE$\downarrow$ & SR$\uparrow$\\
\midrule
Stage 1: episode-level SFT & 52.4 & 48.7 & 58.0 & 5.71 & 56.6\\
Stage 2: + DAgger & 63.7 & 56.7 & 70.6 & 4.23 & 67.2\\
Stage 3: + GRPO~\cite{zhang2026activevln} & 66.8 & 60.0 & 74.4 & 3.85 & 72.4\\
\rowcolor{oursbg}Stage 3: + \core (ours) & \textbf{71.9} & \textbf{63.7} & \textbf{78.6} & \textbf{3.32} & \textbf{73.6}\\
\bottomrule
\end{tabular}\end{adjustbox}


==> tab/speed.tex <==
\caption{\textbf{Inference cost per step} at batch size 1: peak VRAM (GiB) and step time (ms). One step is one policy call (StreamVLN may emit up to four actions per call). Baseline numbers on the two desktop GPUs are from~\cite{dao2026stagevln}; the Jetson numbers are measured with the same protocol. OOM: out of memory (32\,GB; the other devices have 96 and 64\,GB).}
\label{tab:speed}
\setlength{\tabcolsep}{3.1pt}
\footnotesize
\begin{adjustbox}{max width=\linewidth}\begin{tabular}{@{}l cc cc cc@{}}
\toprule
 & \multicolumn{2}{c}{RTX 5090} & \multicolumn{2}{c}{RTX PRO 6000} & \multicolumn{2}{c}{Jetson AGX Orin}\\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(l){6-7}
Method & GiB$\downarrow$ & ms$\downarrow$ & GiB$\downarrow$ & ms$\downarrow$ & GiB$\downarrow$ & ms$\downarrow$\\
\midrule
JanusVLN~\cite{zeng2026janusvln}  & OOM   & OOM   & 35.73 & 481.3 & 35.7 & 7389.8\\
NaVILA~\cite{cheng2024navila}     & 17.47 & 365.2 & 17.47 & 383.1 & 17.5 & 3531.0\\
StreamVLN~\cite{wei2026streamvln} & 17.48 & 233.4 & 17.48 & 209.8 & 17.6 & 2135.5\\
StageVLN~\cite{dao2026stagevln}   & 10.24 & 304.5 & 10.24 & 229.8 & 10.2 & 2175.8\\
\rowcolor{oursbg}\method          & \textbf{8.68} & \textbf{135.7} & \textbf{8.68} & \textbf{103.9} & \textbf{8.9} & \textbf{839.1}\\
\bottomrule
\end{tabular}\end{adjustbox}

